SCORE: Syntactic Code Representations for Static Script Malware Detection

As businesses increasingly adopt cloud technologies, they also need to be aware of new security challenges, such as server-side script attacks, to ensure the integrity of their systems and data. These scripts can steal data, compromise credentials, and disrupt operations. Unlike executables with standardized formats (e.g., ELF, PE), scripts are plaintext files with diverse syntax, making them harder to detect using traditional methods. As a result, more sophisticated approaches are needed to protect cloud infrastructures from these evolving threats. In this paper, we propose novel feature extraction and deep learning (DL)-based approaches for static script malware detection, targeting server-side threats. We extract features from plain-text code using two techniques: syntactic code highlighting (SCH) and abstract syntax tree (AST) construction. SCH leverages complex regexes to parse syntactic elements of code, such as keywords, variable names, etc. ASTs generate a hierarchical representation of a program's syntactic structure. We then propose a sequential and a graph-based model that exploits these feature representations to detect script malware. We evaluate our approach on more than 400K server-side scripts in Bash, Python and Perl. We use a balanced dataset of 90K scripts for training, validation, and testing, with the remaining from 400K reserved for further analysis. Experiments show that our method achieves a true positive rate (TPR) up to 81% higher than leading signature-based antivirus solutions, while maintaining a low false positive rate (FPR) of 0.17%. Moreover, our approach outperforms various neural network-based detectors, demonstrating its effectiveness in learning code maliciousness for accurate detection of script malware.

==> Sections/customer.tex <==
Customers of AWS security products need--and expect--robust protection of their compute infrastructure from malware, and today's malware scanning modules provide that, but with room for improvement. Today's malware detection capability is built primarily atop third-party AV, which are specialized to neither AWS nor the predominantly-Linux-based resources used. As a result, in-house malware detection capabilities can provide maximal value if they specialize to (i) attacks {\it actually observed on AWS customer resources} and (ii) attacks from which customers expect protection.

Findings analytics over the past 11 weeks indicate the relative prevalence of script malware could be as high as 90\% of all malware detected on customer resources; however, this statistic is a best-efforts estimate from limited data visibility, and should be interpreted loosely. Minimally, it suggests a qualitatively high volume of script malware. Against middling antivirus performance on such samples (TPR $\approx$ 0.75, {\it cf.} Table \ref{tab:performance_comparison_all}), there is an urgent performance gap that needs to be bridged to protect our customers. To the best of our knowledge, this research program does not disadvantage, nor pose negative outcomes to, any of those customers.
